Rational terms of UV origin to all loop orders

Numerical approaches to computations typically reconstruct the numerators of Feynman diagrams in four dimensions. In doing so, certain rational terms arising from the (D-4)-dimensional part of the numerator multiplying ultraviolet (UV) poles in dimensional regularisation are not captured and need to be obtained by other means. At one-loop these rational terms of UV origin can be computed from a set of process-independent Feynman rules. Recently, it was shown that this approach can be extended to two loops. In this paper, we show that to all loop orders it is possible to compute rational terms of UV origin through process-independent vertices that are polynomial in masses and momenta.

==> diagram.tex <==
% !TEX root = main.tex

\section{Diagrammatic interpretation of rational $R_2$ terms of UV origin}
\label{sec:diagrams}

In the previous section we have defined the map $\tbR$, which assigns to any amplitude $\cAbar_{\Gamma}$ a polynomial in masses and momenta. It agrees with the rational $R_2$ terms $\delta R_{\Gamma}$ at one and two loops defined in refs.~\cite{Ossola:2008xq,Pozzorini:2020hkx}. However, the lack of multiplicativity of $\tbR$ makes a Feynman diagrammatic interpretation more cumbersome than for the UV counterterms, starting from 1PR graphs at two loops and 1PI graphs at three loops. The goal of this section is to present an alternative definition of counterterm vertices, which combines UV counterterms and $R_2$ vertices into one object, and which has a very clean interpretation in terms of Feynman rules to all orders in perturbation theory.

We start by casting eq.~\eqref{eq:master} in the form
\beq\label{eq:master_U}
\bR\cAbar_{\Gamma} = \sum_{\gamma\in \bW(\Gamma)}\bU\cAbar_{\gamma}\ast\cA_{\Gamma/\gamma}\,.
\eeq 
The map $\bU$ is defined as
\beq
\bU\cAbar_{\gamma} = \tbR\cAbar_{\gamma}  - \bRbar\,\cA_{\gamma}  = \delta R_{\gamma} + \delta Z_{\gamma} \equiv \delta U_{\gamma}\,.
\eeq
Note that eq.~\eqref{eq:master_U} has exactly the same structure as eq.~\eqref{eq:R_to_Rbar}, except that we have replaced $\bR$ and $\cAbar_{\Gamma/\gamma}$ by $\bU$ and $\cA_{\Gamma/\gamma}$.


The map $\bU$ has the following properties:
\begin{enumerate}
\item If $\omega(\Gamma)<0$, then $\bU\,\cAbar_{\Gamma}=0$.
\item $\bU$ commutes with derivatives with respect to external momenta or propagator masses.
\item $\bU\cAbar_{\Gamma}$ is a polynomial in external momenta and propagator masses.
\item $\bU$ is multiplicative:
\beq\bsp\label{eq:U_mult}
\bU\big[\cAbar_{\Gamma_1}\cdot\cAbar_{\Gamma_2}\big]&\, = \bU\cAbar_{\Gamma_1}\cdot\bU\cAbar_{\Gamma_2}\,.
\esp\eeq
\end{enumerate}
The first three properties are a direct consequence of the corresponding properties of $\bRbar$ and $\tbR$. The multiplicativity is new, and we now present the proof.

The proof of eq.~\eqref{eq:U_mult} proceeds by induction in the number of loops. Equation~\eqref{eq:U_mult} is clearly true for one-loop graphs (cf., e.g., eq.~\eqref{eq:fail}).
Assume that $\Gamma=\Gamma_1\Gamma_2$. It is easy to see that $\bW(\Gamma) = \bW(\Gamma_1)\times\bW(\Gamma_2)$. This implies
\beq\bsp\label{eq:mult_1}
\bR\cAbar_{\Gamma}&\, =  \sum_{\gamma_1\in \bW(\Gamma_1)}\sum_{\gamma_2\in \bW(\Gamma_2)}\bU\cAbar_{\gamma_1\gamma_2}\ast\big(\cA_{\Gamma_1/\gamma_1}\,\cA_{\Gamma_2/\gamma_2}\big)\,.
\esp \eeq
We also have
\beq\bsp
\bR\cAbar_{\Gamma_1}\,\bR\cAbar_{\Gamma_2}&\, = \sum_{\gamma_1\in \bW(\Gamma_1)}\sum_{\gamma_2\in \bW(\Gamma_2)}
\big(\bU\cAbar_{\gamma_1}\ast\cA_{\Gamma_1/\gamma_1}\big)\,\big(\bU\cAbar_{\gamma_2}\ast\cA_{\Gamma_2/\gamma_2}\big)\,.
\esp\eeq
We can have a closer look at the terms in the last sum. If we denote the number of loops of $\Gamma_i/\gamma_i$ by $L_i$ ($i=1,2$), we have
\beq\bsp
\big(\bU\cAbar_{\gamma_1}&\ast\cA_{\Gamma_1/\gamma_1}\big)\,\big(\bU\cAbar_{\gamma_2}\ast\cA_{\Gamma_2/\gamma_2}\big) =\\
&\,=
\int\left(\prod_{i=1}^{L_1}\frac{\rd^D\bar{q}_i}{(2\pi)^D}\right)\,\left(\prod_{i=1}^{L_2}\frac{\rd^D\bar{q}'_i}{(2\pi)^D}\right)\,\bU\cAbar_{\gamma_1}\,\bU\cAbar_{\gamma_2}\,\frac{\cN_{\Gamma_1/\gamma_1}\,\cN_{\Gamma_2/\gamma_2}}{\prod_e\overline{D}_e}\\
&\,=
\int\left(\prod_{i=1}^{L_1+L_2}\frac{\rd^D\bar{q}_i}{(2\pi)^D}\right)\,\bU\cAbar_{\gamma_1}\,\bU\cAbar_{\gamma_2}\,\frac{\cN_{\Gamma/(\gamma_1\gamma_2)}}{\prod_e\overline{D}_e}\\
&\,=\big(\bU\cAbar_{\gamma_1}\,\bU\cAbar_{\gamma_2}\big)\ast\cA_{\Gamma/(\gamma_1\gamma_2)}\,,
\esp\eeq
where we used the fact that $\cN_{\Gamma_1/\gamma_1} \cN_{\Gamma_2/\gamma_2} = \cN_{\Gamma/(\gamma_1\gamma_2)}$.
Hence,
\beq\bsp\label{eq:mult_2}
\bR\cAbar_{\Gamma_1}\,\bR\cAbar_{\Gamma_2}&\, =\sum_{\gamma_1\in \bW(\Gamma_1)}\sum_{\gamma_2\in \bW(\Gamma_2)}\big(\bU\cAbar_{\gamma_1}\,\bU\cAbar_{\gamma_2}\big)\ast\cA_{\Gamma/(\gamma_1\gamma_2)}\,.
\esp\eeq
Taking the difference between eqs.~\eqref{eq:mult_1} and~\eqref{eq:mult_2}, we see that all terms cancel, except the one for $(\gamma_1,\gamma_2)=(\Gamma_1,\Gamma_2)$, and we recover eq.~\eqref{eq:U_mult}.

As the map $\bU$ satisfies the same properties as the map $\bRbar$ used to define UV counterterms, eq.~\eqref{eq:master_U} has a direct interpretation in terms of Feynman diagrams, just like for UV renormalisation: The renormalised Feynman diagram $\bR\cAbar_{\Gamma}$ is obtained by adding to $\cA_{\Gamma}$ all Feynman diagrams obtained by replacing a superficially divergent 1PI graph $\gamma$ by the tree-level vertex $\delta U_{\gamma}$, which is a polynomial in masses and momenta. We can split $\delta U_{\gamma} = \delta Z_{\gamma} + \delta R_{\gamma}$, and these Feynman diagrams can be grouped into three classes:
\begin{itemize}
\item Diagrams with only UV counterterm vertices $\delta Z_{\gamma}$ inserted: those correspond precisely to the UV counterterms introduced by the BPHZ formula.
\item Diagrams with only $R_2$ vertices $\delta R_{\gamma}$ inserted.
\item  Diagrams with both UV counterterms and $R_2$ vertices inserted. Those diagrams appear for the first time for 1PR diagrams at two loops, and 1PI diagrams at three loops.
\end{itemize}



==> rational.tex <==
% !TEX root = main.tex

\section{Rational terms of UV origin}
\label{sec:R2}

\subsection{All-order definition of rational terms of UV origin}

In this section we present our definition of rational $R_2$ terms of UV origin at all loop orders. We start by recursively defining a map $\tbR$:
\beq\label{eq:Rtilde}
\tbR\cAbar_{\Gamma} =\bF\Bigg[\bR\cAbar_{\Gamma}  - \bR\cA_{\Gamma}  -\sum_{\gamma\in W(\Gamma)}\tbR\cAbar_{\gamma}\ast \cA_{\Gamma/\gamma}\Bigg]\,.
\eeq
The recursion starts with $\tbR\cAbar_{\Gamma} =\bR\cAbar_{\Gamma}  - \bR\cAbar_{\Gamma}$ if $\Gamma$ is a one-loop graph (because a one-loop graph does not have any proper 1PI subgraphs). The operator $\bF$ is similar to $\bK$, but it extracts in addition the coefficient of $\eps^0$:
\beq
\bF\big[f(\eps)\big] = \eps\,\bK\big[\eps^{-1}\,f(\eps)\big]\,.
\eeq
In the MS and $\MS$-schemes it is explicitly given by
\beq
\bF_{\textrm{MS}}\big[f(\eps)\big] = \sum_{k=k_0}^0f_k\,\eps^k \textrm{~~~and~~~}
\bF_{{\MS}}\big[f(\eps)\big] = \bF_{\textrm{MS}}\big[(4\pi)^{L\eps}e^{\gamma_E\eps}f(\eps)\big]\,.
\eeq
Note that $\tbR$ depends on the choice of the renormalisation scheme, through the explicit appearance of the renormalised amplitudes.

Equation~\eqref{eq:Rtilde} can be cast in the form
\beq\label{eq:master}
\bR\cAbar_{\Gamma} - \bR\cA_{\Gamma} = \tbR\cAbar_{\Gamma} +\sum_{\gamma\in W(\Gamma)}\tbR\cAbar_{\gamma}\ast \cA_{\Gamma/\gamma} + \ord(\eps)\,,
\eeq
where we used the fact that $\bF[f(\eps)]= f(\eps)+\ord(\eps)$. 
We see that the $\tbR$ map allows us to compute the finite terms from the difference of the renormalised amplitudes $\bR\cAbar_{\Gamma} - \bR\cA_{\Gamma}$. 

We start by stating the following properties of the map $\tbR$:
\begin{enumerate}
\item If $\omega(\Gamma)<0$, then $\tbR\,\cAbar_{\Gamma}=0$.
\item $\tbR$ commutes with derivatives with respect to external momenta or propagator masses.
\item $\tbR\cAbar_{\Gamma}$ is a polynomial in external momenta and propagator masses.
\end{enumerate}
Note that these three properties are the analogues of the first three properties of the $\bRbar$ map reviewed in the previous section. Also note that we can extract the poles of $\tbR\cAbar_{\Gamma}$ by acting with $\bK$. Since $\bK\bR=0$ and $\bK\bF=\bK$, we find
\beq
\bK\tbR\cAbar_{\Gamma} = -\bK\Bigg[\sum_{\gamma\in W(\Gamma)}\tbR\cAbar_{\gamma}\ast \cA_{\Gamma/\gamma}\Bigg]\,.
\eeq
We see that the poles of $\tbR\cAbar_{\Gamma} $ are entirely determined by lower-loop information. In particular, if $\Gamma$ is a one-loop graph, $\bK\tbR\cAbar_{\Gamma} = 0$. Starting from two loops, $\tbR\cAbar_{\Gamma} $ will in general contain poles in $\eps$.

So far, eq.~\eqref{eq:master} is simply a recasting of the definition in eq.~\eqref{eq:Rtilde}. In the remainder of this section, we show that the right-hand side of eq.~\eqref{eq:master} can be interpreted as the generalisation of the one- and two-loop definition of the $R_2$ vertices reviewed in the previous section. 
Let us now show that $\tbR\cAbar_{\Gamma}$ agrees with the one- and two-loop $R_2$ vertices $\delta R_{\Gamma}$ defined in refs.~\cite{Ossola:2008xq,Pozzorini:2020hkx}. First, Properties 1 and 3 imply that $\tbR\cAbar_{\Gamma}$ is non-zero only for superficially divergent graphs, and it is polynomial in masses and momenta. At one-loop, we obtain:
\beq
\tbR\cAbar_{\Gamma} = \bR\cAbar_{\Gamma} - \bR\cA_{\Gamma} = \cAbar_{\Gamma} - \cA_{\Gamma} = \delta R_{\Gamma}+\ord(\eps)\,,
\eeq
where the second equality follows from the fact that in the HV scheme, the one-loop UV counterterms for $\cAbar_{\Gamma}$ and $\cA_{\Gamma}$ are identical. At two-loop order, eq.~\eqref{eq:master} reduces to
\beq\bsp
\bR\cAbar_{\Gamma} 
&\,= \cA_{\Gamma} +\delta Z_{\Gamma} + \tbR\cAbar_{\Gamma} +\sum_{\gamma\in W(\gamma)}(\tbR\cAbar_{\gamma} +\delta Z_{\gamma})\ast \cA_{\Gamma/\gamma}+\ord(\eps)\\
&\,= \cA_{\Gamma} +\delta Z_{\Gamma} + \tbR\cAbar_{\Gamma} +\sum_{\gamma\in W(\gamma)}(\delta R_\gamma+\delta Z_{\gamma})\ast \cA_{\Gamma/\gamma}+\ord(\eps)\,.
\esp\eeq
Comparing to eq.~\eqref{eq:two-loop-R2-master}, we see that we have $\delta R_\Gamma = \tbR\cAbar_{\Gamma}$.






Unlike $\bR$ and $\bRbar$, the map $\tbR$ is not multiplicative. This effect did not arise in the two-loop discussion of ref.~\cite{Pozzorini:2020hkx}, because for two-loop 1PI graphs, there are no subdiagrams that are disconnected 1PI graphs. The non-multiplicativity of $\tbR$ comes into play for the first time at three loops for 1PI graphs, and at two loops for 1PR graphs. For example, if $\Gamma=\Gamma_1\Gamma_2$ is a disconnected two-loop graph which is a product of two one-loop graphs, we have
\beq\bsp
\bR\big[\cAbar_{\Gamma_1}\,\cAbar_{\Gamma_2}\big] &\,= \bR\cAbar_{\Gamma_1}\,\bR\cAbar_{\Gamma_2}\\
&=\left(\bR\cA_{\Gamma_1}+\tbR\cAbar_{\Gamma_1}\right)\,\left(\bR\cA_{\Gamma_2}+\tbR\cAbar_{\Gamma_2}\right)+\ord(\eps)\\
&=\bR\cA_{\Gamma_1}\,\bR\cA_{\Gamma_2}+\tbR\cAbar_{\Gamma_1}\cA_{\Gamma_2}+\tbR\cAbar_{\Gamma_2}\cA_{\Gamma_1}\\
&\, \phantom{=}+ \tbR\cAbar_{\Gamma_1}\,\tbR\cAbar_{\Gamma_2}- \tbR\cAbar_{\Gamma_1}\,\bRbar\,\cAbar_{\Gamma_2}- \bRbar\,\cAbar_{\Gamma_1}\,\tbR\cAbar_{\Gamma_2}+\ord(\eps)\,.
\esp\eeq
From this we see that
\beq\bsp\label{eq:fail}
\tbR\big[\cAbar_{\Gamma_1}\,\cAbar_{\Gamma_2}\big] &\,=  \tbR\cAbar_{\Gamma_1}\,\tbR\cAbar_{\Gamma_2}- \tbR\cAbar_{\Gamma_1}\,\bRbar\,\cAbar_{\Gamma_2}- \bRbar\,\cAbar_{\Gamma_1}\,\tbR\cAbar_{\Gamma_2} \\
&\,\neq
\tbR\cAbar_{\Gamma_1}\,\tbR\cAbar_{\Gamma_2}\,.
\esp\eeq
The lack of multiplicativity makes a Feynman diagrammatic interpretation of $R_2$ vertices less straightforward than for the UV divergences. We will return to this point in section~\ref{sec:diagrams}.

Finally, we need to comment on IR divergencies. Strictly speaking, our derivation only holds in the absence of IR divergencies. It is only proven that rational $R_2$ terms of IR origin cancel at one loop in the HV scheme
at the level of the full amplitude~\cite{Bredenstein:2008zb}. In a theory with IR divergencies, in particular massless gauge theories, we may still use the $\tbR$ map to extract the contribution to the rational $R_2$ terms that are of UV origin. In order to isolate those UV contributions, we may, e.g., proceed as in ref.~\cite{Pozzorini:2020hkx} and apply a tadpole decomposition~\cite{Misiak:1994zw,Chetyrkin:1997fm} to the integrand. This results in a sum of integrals with massive propagators, which are free of IR divergencies, and a contribution with negative superficial degree of divergence, which does not contribute to the $R_2$ terms of UV origin due to Property 2 form the theorem. In this way we can isolate the UV divergent contributions to an integral, and extract the corresponding rational $R_2$ terms using the $\tbR$ map.











